A Personalized Federated Learning Algorithm: an Application in Anomaly Detection

Federated Learning (FL) has recently emerged as a promising method that employs a distributed learning model structure to overcome data privacy and transmission issues paused by central machine learning models. In FL, datasets collected from different devices or sensors are used to train local models (clients) each of which shares its learning with a centralized model (server). However, this distributed learning approach presents unique learning challenges as the data used at local clients can be non-IID (Independent and Identically Distributed) and statistically diverse which decrease learning accuracy in the central model. In this paper, we overcome this problem by proposing a novel Personalized Conditional FedAvg (PC-FedAvg) which aims to control weights communication and aggregation augmented with a tailored learning algorithm to personalize the resulting models at each client. Our experimental validation on two datasets showed that our PC-FedAvg precisely constructed generalized clients' models and thus achieved higher accuracy compared to other state-of-the-art methods.

==> background.tex <==
\section{Background}

\subsection{One-Class Support Vector Machine}
\label{s:ocsvm}

Given a set of data $X=\{{x_i}\}_{i=1}^n$, $n$ is the number of training samples, OCSVM maps these samples into a high dimensional feature space using  function  $\phi$ through  the kernel $K(x_i,x_j) = \phi(x_i)^T \phi(x_j)$. Then OCSVM tries to learn a decision boundary that maximally separates the training samples from the origin \cite{scholkopf2001estimating}. The primary objective of OCSVM   is to optimize  the  following equation:
\begin{eqnarray}\label{ocsvm}
	\min_{w,\xi,\rho}  \frac{1}{2} \lVert w \rVert^{2} 	+ \frac{1}{\nu n} \sum_{i=1}^n \xi_i - \rho
\end{eqnarray}
\begin{eqnarray*}
	s.t \hspace{2em}  w. \phi(x_i) \geq \rho - \xi_i,\hspace{1em}   \xi_i \geq 0, \hspace{1em}  i = 1, \ldots, n.     
\end{eqnarray*}
where $ 0< \nu < 0$ is a user defined parameter used to control the rate of anomalies in the training data, $\xi$ are the slack variables,  $w$ is a perpendicular vector to the decision boundary and $\rho$ known as  the bias term. 
To solve this  dual problem, we  introduce the   Lagrangian  multipliers $\alpha_i, \alpha_j \geq 0$ in the loss function defines as:

\begin{eqnarray}\label{lag}
	L_{(w,\xi,\rho, \alpha_i, \alpha_j)}  =   \frac{1}{2} \lVert w \rVert^{2} 	+ \frac{1}{\nu n} \sum_{i=1}^n \xi_i - \rho
	- \sum_{i=1}^n \alpha_i ((w.\phi(x_i)) - \rho + \xi_i) -  \sum_{j=1}^n \alpha_j \xi_j
\end{eqnarray}

Taking the derivative of $L$ with respect to the primal variables $w,\xi,\rho $  and setting those to zero, we obtain

\begin{eqnarray}\label{dw}
	\frac{dL(w,\xi,\rho, \alpha_i, \alpha_j)}{dw}  =    w - \sum_{i=1}^n \alpha_i \phi(x_i ) = 0
\end{eqnarray}
\begin{eqnarray}\label{dxi}
	\frac{dL(w,\xi,\rho, \alpha_i, \alpha_j)}{d\xi}  =   \frac{1}{\nu n} -  \alpha_i - \alpha_j = 0
\end{eqnarray}
\begin{eqnarray}\label{db}
	\frac{dL(w,\xi,\rho, \alpha_i, \alpha_j)}{d\rho}  =  -1 + \sum_{i=1}^n \alpha_i = 0
\end{eqnarray}

From Equations \ref{dw}, \ref{dxi},\ref{db}, we can get 
\begin{eqnarray}\label{dw2}
	   w = \sum_{i=1}^n \alpha_i \phi(x_i ) 
\end{eqnarray}
\begin{eqnarray}\label{dxi2}
 	 \alpha_i = \frac{1}{\nu n} - \alpha_j 
\end{eqnarray}
\begin{eqnarray}\label{db2}
	\sum_{i=1}^n \alpha_i = 1
\end{eqnarray}



Substituting Equations \ref{dw2} and \ref{dxi2} into equation \ref{lag}, and using a kernel function method $K(x_i,x_j) = \phi(x_i)^T \phi(x_j)$, we obtain the dual problem:

\begin{eqnarray}\label{cost}
\max J(\alpha) = \sum_{i}^n\alpha_i -  \frac{1}{2}\sum_{i}^n \sum_{j}^n \alpha_i\alpha_j K(x_i, x_j)
\end{eqnarray}

\begin{eqnarray*}
	s.t \hspace{2em} 0 \leq \alpha_i \leq \frac{1}{\nu n},\hspace{1em} \sum_{i=1}^n    \alpha_i =1,
\end{eqnarray*}
where $ K(x_i, x_j)$ is the kernel matrix and $\alpha$ are the Lagrange multipliers.


After we obtain the solution $\alpha$ of the dual optimization problem, all patterns ${x_i: i \in [l],\alpha_i > 0 } $ are called support vectors. The decision function to compute the anomaly score for  a query  sample $x$ is  defined as:

\begin{eqnarray}\label{dg}
	g(x) =     \sum_{i=1}^{n_s}\alpha_i K(x_i, x)-\rho.
\end{eqnarray}

The variable $\rho$ can be  calculated by exploiting any such $\alpha_i > 0$ for its corresponding  pattern $x_i$ as follows:

\begin{eqnarray}\label{rho}
 \rho =     \sum_{j=1}^{n}\alpha_j K(x_, x_i)-\rho.
\end{eqnarray}

The OCSVM will use Equation \ref{df} to identify whether a query point  belongs to the positive class when returning a positive value and 	vice versa if it generates a negative value.

\begin{eqnarray}\label{df}
	f(x) = sgn(g(x))
\end{eqnarray}




==> setup.tex <==
\section{Experimental Setup}
\label{s:setup}

